Adversarial Robustness of Bottleneck Injected Deep Neural Networks for Task-Oriented Communication

This paper investigates the adversarial robustness of Deep Neural Networks (DNNs) using Information Bottleneck (IB) objectives for task-oriented communication systems. We empirically demonstrate that while IB-based approaches provide baseline resilience against attacks targeting downstream tasks, the reliance on generative models for task-oriented communication introduces new vulnerabilities. Through extensive experiments on several datasets, we analyze how bottleneck depth and task complexity influence adversarial robustness. Our key findings show that Shallow Variational Bottleneck Injection (SVBI) provides less adversarial robustness compared to Deep Variational Information Bottleneck (DVIB) approaches, with the gap widening for more complex tasks. Additionally, we reveal that IB-based objectives exhibit stronger robustness against attacks focusing on salient pixels with high intensity compared to those perturbing many pixels with lower intensity. Lastly, we demonstrate that task-oriented communication systems that rely on generative models to extract and recover salient information have an increased attack surface. The results highlight important security considerations for next-generation communication systems that leverage neural networks for goal-oriented compression.

==> embed/tables/_tab_resilience_all.tex <==
\begin{table}[htb]
\setlength{\tabcolsep}{4pt}
\caption{Adversarial Resilience on CIFAR-10}
\label{tab:resilience_all}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llrrr|rrr|rrr}
%\hline
                             &                              & \multicolumn{3}{c}{CIFAR-10}       &  \multicolumn{3}{c}{SVHN}          & \multicolumn{3}{c}{ImageNet64} \\ \hline
Model                        & Attack                       & Base & SVBI & DVBI & Base & SVBI & DVBI & Base & SVBI & DVBI \\ \hline
                             & FGSM                         & 74.56                              & 48.75                              & 39.52                              & 69.95                         & 51.54                         & 42.31                         & 37.76                              & 32.72                              & 28.59                              \\
                             & \cellcolor[HTML]{EFEFEF}EAD  & \cellcolor[HTML]{EFEFEF}85.52      & \cellcolor[HTML]{EFEFEF}3.64       & \cellcolor[HTML]{EFEFEF}2.85       & \cellcolor[HTML]{EFEFEF}90.54 & \cellcolor[HTML]{EFEFEF}8.34  & \cellcolor[HTML]{EFEFEF}7.36  & \cellcolor[HTML]{EFEFEF}35.43      & \cellcolor[HTML]{EFEFEF}1.96       & \cellcolor[HTML]{EFEFEF}1.13       \\
                             & C\&W                         & 87.01                              & 7.77                               & 4.76                               & 92.37                         & 13.67                         & 12.86                         & 37.85                              & 5.48                               & 1.196                              \\
\multirow{-4}{*}{ResNet-18}  & \cellcolor[HTML]{EFEFEF}JSMA & \cellcolor[HTML]{EFEFEF}87.62      & \cellcolor[HTML]{EFEFEF}20.78      & \cellcolor[HTML]{EFEFEF}17.57      & \cellcolor[HTML]{EFEFEF}93.58 & \cellcolor[HTML]{EFEFEF}21.73 & \cellcolor[HTML]{EFEFEF}18.41 & \cellcolor[HTML]{EFEFEF}34.66      & \cellcolor[HTML]{EFEFEF}17.07      & \cellcolor[HTML]{EFEFEF}9.00       \\ \hline
                             & FGSM                         & 68.85                              & 37.84                              & 24.72                              & 58.06                         & 49.48                         & 42.09                         & 41.70                              & 32.22                              & 32.18                              \\
                             & \cellcolor[HTML]{EFEFEF}EAD  & \cellcolor[HTML]{EFEFEF}85.14      & \cellcolor[HTML]{EFEFEF}4.61       & \cellcolor[HTML]{EFEFEF}4.52       & \cellcolor[HTML]{EFEFEF}92.09 & \cellcolor[HTML]{EFEFEF}9.83  & \cellcolor[HTML]{EFEFEF}7.23  & \cellcolor[HTML]{EFEFEF}37.73      & \cellcolor[HTML]{EFEFEF}1.81       & \cellcolor[HTML]{EFEFEF}1.15       \\
                             & C\&W                         & 88.01                              & 6.56                               & 5.42                               & 88.78                         & 10.20                         & 12.08                         & 41.73                              & 5.52                               & 2.56                               \\
\multirow{-4}{*}{ResNet-50}  & \cellcolor[HTML]{EFEFEF}JSMA & \cellcolor[HTML]{EFEFEF}85.10      & \cellcolor[HTML]{EFEFEF}19.63      & \cellcolor[HTML]{EFEFEF}17.87      & \cellcolor[HTML]{EFEFEF}90.17 & \cellcolor[HTML]{EFEFEF}20.22 & \cellcolor[HTML]{EFEFEF}16.08 & \cellcolor[HTML]{EFEFEF}39.32      & \cellcolor[HTML]{EFEFEF}19.18      & \cellcolor[HTML]{EFEFEF}10.25      \\ \hline
                             & FGSM                         & 69.31                              & 37.84                              & 34.08                              & 68.31                         & 44.94                         & 45.59                         & 41.71                              & 31.13                              & 30.12                              \\
                             & \cellcolor[HTML]{EFEFEF}EAD  & \cellcolor[HTML]{EFEFEF}88.65      & \cellcolor[HTML]{EFEFEF}4.61       & \cellcolor[HTML]{EFEFEF}4.52       & \cellcolor[HTML]{EFEFEF}94.32 & \cellcolor[HTML]{EFEFEF}9.78  & \cellcolor[HTML]{EFEFEF}8.96  & \cellcolor[HTML]{EFEFEF}41.66      & \cellcolor[HTML]{EFEFEF}1.84       & \cellcolor[HTML]{EFEFEF}1.04       \\
                             & C\&W                         & 87.75                              & 6.56                               & 5.42                               & 93.23                         & 12.48                         & 11.85                         & 41.94                              & 5.53                               & 2.53                               \\
\multirow{-4}{*}{ResNet-100} & \cellcolor[HTML]{EFEFEF}JSMA & \cellcolor[HTML]{EFEFEF}83.58      & \cellcolor[HTML]{EFEFEF}19.63      & \cellcolor[HTML]{EFEFEF}17.87      & \cellcolor[HTML]{EFEFEF}94.08 & \cellcolor[HTML]{EFEFEF}19.39 & \cellcolor[HTML]{EFEFEF}18.03 & \cellcolor[HTML]{EFEFEF}38.97      & \cellcolor[HTML]{EFEFEF}15.39      & \cellcolor[HTML]{EFEFEF}11,12      \\ \hline
\end{tabular}%
}
\end{table}


==> embed/tables/tab_degredation_params.tex <==
\begin{table}[htb]
\centering
\caption{Degredation Parameters Applied to Different Datasets}
\begin{tabular}{|l|c|c|c|c|}
\hline
\textbf{Dataset} & \textbf{Gaussian Noise} & \textbf{Defocus Blur} & \textbf{Motion Blur} & \textbf{Low Contrast} \\ \hline
MNIST      & SD: 0.5 & Radius: 1.5 & 5x5 Kernel & Factor: 0.1 \\ \hline
CIFAR-10   & SD: 0.025 & Radius: 2.0 & 5x5 Kernel & Factor: 0.25 \\ \hline
SVHN       & SD: 0.025 & Radius: 2.0 & 5x5 Kernel & Factor: 0.25 \\ \hline
ImageNet64 & SD: 0.1 & Radius: 1.25 & 5x5 Kernel & Factor: 0.75 \\ \hline
Felidae    & SD: 0.1 & Radius: 2.0 & 5x5 Kernel & Factor: 0.5 \\ \hline
\end{tabular}
\label{tab:degredations}
\end{table}

==> embed/tables/tab_resilience_all_2col.tex <==
\begin{table*}[htb]
%\setlength{\tabcolsep}{12pt}
\caption{Comparing Adversarial Robustness between Objectives}
\label{tab:resilience_all}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llrrr|rrr|rrr}
%\hline
                             &                              & \multicolumn{3}{c}{CIFAR-10}       &  \multicolumn{3}{c}{SVHN}          & \multicolumn{3}{c}{ImageNet64} \\ \hline
Model                        & Attack                       & Base & SVBI & DVBI & Base & SVBI & DVBI & Base & SVBI & DVBI \\ \hline
                             & FGSM                         & 74.5600                              & 48.7500                              & 39.5200                              & 69.9500                         & 51.5400                         & 42.3100                         & 37.7600                              & 32.7200                              & 28.5900                              \\
                             & \cellcolor[HTML]{EFEFEF}EAD  & \cellcolor[HTML]{EFEFEF}85.52      & \cellcolor[HTML]{EFEFEF}3.64       & \cellcolor[HTML]{EFEFEF}2.85       & \cellcolor[HTML]{EFEFEF}90.54 & \cellcolor[HTML]{EFEFEF}8.34  & \cellcolor[HTML]{EFEFEF}7.36  & \cellcolor[HTML]{EFEFEF}35.43      & \cellcolor[HTML]{EFEFEF}1.96       & \cellcolor[HTML]{EFEFEF}1.13       \\
                             & C\&W                         & 87.01                              & 7.77                               & 4.76                               & 92.37                         & 13.67                         & 12.86                         & 37.85                              & 5.48                               & 1.196                              \\
\multirow{-4}{*}{ResNet-18}  & \cellcolor[HTML]{EFEFEF}JSMA & \cellcolor[HTML]{EFEFEF}87.62      & \cellcolor[HTML]{EFEFEF}20.78      & \cellcolor[HTML]{EFEFEF}17.57      & \cellcolor[HTML]{EFEFEF}93.58 & \cellcolor[HTML]{EFEFEF}21.73 & \cellcolor[HTML]{EFEFEF}18.41 & \cellcolor[HTML]{EFEFEF}34.66      & \cellcolor[HTML]{EFEFEF}17.07      & \cellcolor[HTML]{EFEFEF}9.00       \\ \hline
                             & FGSM                         & 68.85                              & 37.84                              & 24.72                              & 58.06                         & 49.48                         & 42.09                         & 41.70                              & 32.22                              & 32.18                              \\
                             & \cellcolor[HTML]{EFEFEF}EAD  & \cellcolor[HTML]{EFEFEF}85.14      & \cellcolor[HTML]{EFEFEF}4.61       & \cellcolor[HTML]{EFEFEF}4.52       & \cellcolor[HTML]{EFEFEF}92.09 & \cellcolor[HTML]{EFEFEF}9.83  & \cellcolor[HTML]{EFEFEF}7.23  & \cellcolor[HTML]{EFEFEF}37.73      & \cellcolor[HTML]{EFEFEF}1.81       & \cellcolor[HTML]{EFEFEF}1.15       \\
                             & C\&W                         & 88.01                              & 6.56                               & 5.42                               & 88.78                         & 10.20                         & 12.08                         & 41.73                              & 5.52                               & 2.56                               \\
\multirow{-4}{*}{ResNet-50}  & \cellcolor[HTML]{EFEFEF}JSMA & \cellcolor[HTML]{EFEFEF}85.10      & \cellcolor[HTML]{EFEFEF}19.63      & \cellcolor[HTML]{EFEFEF}17.87      & \cellcolor[HTML]{EFEFEF}90.17 & \cellcolor[HTML]{EFEFEF}20.22 & \cellcolor[HTML]{EFEFEF}16.08 & \cellcolor[HTML]{EFEFEF}39.32      & \cellcolor[HTML]{EFEFEF}19.18      & \cellcolor[HTML]{EFEFEF}10.25      \\ \hline
                             & FGSM                         & 69.31                              & 37.84                              & 34.08                              & 68.31                         & 44.94                         & 45.59                         & 41.71                              & 31.13                              & 30.12                              \\
                             & \cellcolor[HTML]{EFEFEF}EAD  & \cellcolor[HTML]{EFEFEF}88.65      & \cellcolor[HTML]{EFEFEF}4.61       & \cellcolor[HTML]{EFEFEF}4.52       & \cellcolor[HTML]{EFEFEF}94.32 & \cellcolor[HTML]{EFEFEF}9.78  & \cellcolor[HTML]{EFEFEF}8.96  & \cellcolor[HTML]{EFEFEF}41.66      & \cellcolor[HTML]{EFEFEF}1.84       & \cellcolor[HTML]{EFEFEF}1.04       \\
                             & C\&W                         & 87.75                              & 6.56                               & 5.42                               & 93.23                         & 12.48                         & 11.85                         & 41.94                              & 5.53                               & 2.53                               \\
\multirow{-4}{*}{ResNet-101} & \cellcolor[HTML]{EFEFEF}JSMA & \cellcolor[HTML]{EFEFEF}83.58      & \cellcolor[HTML]{EFEFEF}19.63      & \cellcolor[HTML]{EFEFEF}17.87      & \cellcolor[HTML]{EFEFEF}94.08 & \cellcolor[HTML]{EFEFEF}19.39 & \cellcolor[HTML]{EFEFEF}18.03 & \cellcolor[HTML]{EFEFEF}38.97      & \cellcolor[HTML]{EFEFEF}15.39      & \cellcolor[HTML]{EFEFEF}11,12      \\ \hline
\end{tabular}%
}
\end{table*}


==> embed/tables/tab_resilience_cifar.tex <==
\begin{table}[htb]
\caption{Adversarial Resilience on CIFAR-10}
\label{tab:resilience_cifar}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llrrr}
Model                        & Attack                       & \multicolumn{1}{l}{Base {[}-\%{]}} & \multicolumn{1}{l}{SVBI {[}-\%{]}} & \multicolumn{1}{l}{DVBI {[}-\%{]}} \\ \hline
                             & FGSM                         & 74.56                              & 48.75                              & 39.52                              \\
                             & \cellcolor[HTML]{EFEFEF}EAD  & \cellcolor[HTML]{EFEFEF}85.52      & \cellcolor[HTML]{EFEFEF}3.64       & \cellcolor[HTML]{EFEFEF}2.85       \\
                             & C\&W                         & 87.01                              & 7.77                               & 4.76                               \\
\multirow{-4}{*}{ResNet-18}  & \cellcolor[HTML]{EFEFEF}JSMA & \cellcolor[HTML]{EFEFEF}87.62      & \cellcolor[HTML]{EFEFEF}20.78      & \cellcolor[HTML]{EFEFEF}17.57      \\ \hline
                             & FGSM                         & 68.85                              & 37.84                              & 24.72                              \\
                             & \cellcolor[HTML]{EFEFEF}EAD  & \cellcolor[HTML]{EFEFEF}85.14      & \cellcolor[HTML]{EFEFEF}4.61       & \cellcolor[HTML]{EFEFEF}4.52       \\
                             & C\&W                         & 88.01                              & 6.56                               & 5.42                               \\
\multirow{-4}{*}{ResNet-50}  & \cellcolor[HTML]{EFEFEF}JSMA & \cellcolor[HTML]{EFEFEF}85.10      & \cellcolor[HTML]{EFEFEF}19.63      & \cellcolor[HTML]{EFEFEF}17.87      \\ \hline
                             & FGSM                         & 69.31                              & 37.84                              & 34.08                              \\
                             & \cellcolor[HTML]{EFEFEF}EAD  & \cellcolor[HTML]{EFEFEF}88.65      & \cellcolor[HTML]{EFEFEF}4.61       & \cellcolor[HTML]{EFEFEF}4.52       \\
                             & C\&W                         & 87.75                              & 6.56                               & 5.42                               \\
\multirow{-4}{*}{ResNet-101} & \cellcolor[HTML]{EFEFEF}JSMA & \cellcolor[HTML]{EFEFEF}83.58      & \cellcolor[HTML]{EFEFEF}19.63      & \cellcolor[HTML]{EFEFEF}17.87      \\ \hline
\end{tabular}%
}
\end{table}

==> embed/tables/tab_resilience_imagenet.tex <==
\begin{table}[htb]
\caption{Adversarial Resilience on ImageNet64}
\label{tab:resilience_imagenet64}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llrrr}
Model                        & Attack                       & \multicolumn{1}{l}{Base {[}-\%{]}} & \multicolumn{1}{l}{SVBI {[}-\%{]}} & \multicolumn{1}{l}{DVBI {[}-\%{]}} \\ \hline
                             & FGSM                         & 37.76                              & 32.72                              & 28.59                              \\
                             & \cellcolor[HTML]{EFEFEF}EAD  & \cellcolor[HTML]{EFEFEF}35.43      & \cellcolor[HTML]{EFEFEF}1.96       & \cellcolor[HTML]{EFEFEF}1.13       \\
                             & C\&W                         & 37.85                              & 5.48                               & 1.196                              \\
\multirow{-4}{*}{ResNet-18}  & \cellcolor[HTML]{EFEFEF}JSMA & \cellcolor[HTML]{EFEFEF}34.66      & \cellcolor[HTML]{EFEFEF}17.07      & \cellcolor[HTML]{EFEFEF}9.00       \\ \hline
                             & FGSM                         & 41.70                              & 32.22                              & 32.18                              \\
                             & \cellcolor[HTML]{EFEFEF}EAD  & \cellcolor[HTML]{EFEFEF}37.73      & \cellcolor[HTML]{EFEFEF}1.81       & \cellcolor[HTML]{EFEFEF}1.15       \\
                             & C\&W                         & 41.73                              & 5.52                               & 2.56                               \\
\multirow{-4}{*}{ResNet-50}  & \cellcolor[HTML]{EFEFEF}JSMA & \cellcolor[HTML]{EFEFEF}39.32      & \cellcolor[HTML]{EFEFEF}19.18      & \cellcolor[HTML]{EFEFEF}10.25      \\ \hline
                             & FGSM                         & 41.71                              & 31.13                              & 30.12                              \\
                             & \cellcolor[HTML]{EFEFEF}EAD  & \cellcolor[HTML]{EFEFEF}41.66      & \cellcolor[HTML]{EFEFEF}1.84       & \cellcolor[HTML]{EFEFEF}1.04       \\
                             & C\&W                         & 41.94                              & 5.53                               & 2.53                               \\
\multirow{-4}{*}{ResNet-101} & \cellcolor[HTML]{EFEFEF}JSMA & \cellcolor[HTML]{EFEFEF}38.97      & \cellcolor[HTML]{EFEFEF}15.39      & \cellcolor[HTML]{EFEFEF}11,12      \\ \hline
\end{tabular}%
}
\end{table}

==> embed/tables/tab_resilience_svhn.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\caption{Adversarial Resilience on SVHN}
\label{tab:resilience_svhn}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llrrr}
Model                        & Attack                       & Base  {[}-\%{]}               & SVBI {[}-\%{]}                & DVBI {[}-\%{]}                \\ \hline
                             & FGSM                         & 69.95                         & 51.54                         & 42.31                         \\
                             & \cellcolor[HTML]{EFEFEF}EAD  & \cellcolor[HTML]{EFEFEF}90.54 & \cellcolor[HTML]{EFEFEF}8.34  & \cellcolor[HTML]{EFEFEF}7.36  \\
                             & C\&W                         & 92.37                         & 13.67                         & 12.86                         \\
\multirow{-4}{*}{ResNet-18}  & \cellcolor[HTML]{EFEFEF}JSMA & \cellcolor[HTML]{EFEFEF}93.58 & \cellcolor[HTML]{EFEFEF}21.73 & \cellcolor[HTML]{EFEFEF}18.41 \\ \hline
                             & FGSM                         & 58.06                         & 49.48                         & 42.09                         \\
                             & \cellcolor[HTML]{EFEFEF}EAD  & \cellcolor[HTML]{EFEFEF}92.09 & \cellcolor[HTML]{EFEFEF}9.83  & \cellcolor[HTML]{EFEFEF}7.23  \\
                             & C\&W                         & 88.78                         & 10.20                         & 12.08                         \\
\multirow{-4}{*}{ResNet-50}  & \cellcolor[HTML]{EFEFEF}JSMA & \cellcolor[HTML]{EFEFEF}90.17 & \cellcolor[HTML]{EFEFEF}20.22 & \cellcolor[HTML]{EFEFEF}16.08 \\ \hline
                             & FGSM                         & 68.31                         & 44.94                         & 45.59                         \\
                             & \cellcolor[HTML]{EFEFEF}EAD  & \cellcolor[HTML]{EFEFEF}94.32 & \cellcolor[HTML]{EFEFEF}9.78  & \cellcolor[HTML]{EFEFEF}8.96  \\
                             & C\&W                         & 93.23                         & 12.48                         & 11.85                         \\
\multirow{-4}{*}{ResNet-101} & \cellcolor[HTML]{EFEFEF}JSMA & \cellcolor[HTML]{EFEFEF}94.08 & \cellcolor[HTML]{EFEFEF}19.39 & \cellcolor[HTML]{EFEFEF}18.03 \\ \hline
\end{tabular}%
}
\end{table}
